A Randomized Rounding Algorithm for Sparse PCA

We present and analyze a simple, two-step algorithm to approximate the optimal solution of the sparse PCA problem. Our approach first solves a L1 penalized version of the NP-hard sparse PCA optimization problem and then uses a randomized rounding strategy to sparsify the resulting dense solution. Our main theoretical result guarantees an additive error approximation and provides a tradeoff between sparsity and accuracy. Our experimental evaluation indicates that our approach is competitive in practice, even compared to state-of-the-art toolboxes such as Spasm.

==> title_abstract.tex <==
\title{A Randomized Rounding Algorithm for Sparse PCA}

\author{
Kimon Fountoulakis
\thanks{
School of Mathematics,
University of Edinburgh,
Edinburgh, UK, K.Fountoulakis@sms.ed.ac.uk.
}
\and
Abhisek Kundu
\thanks{
Department of Computer Science,
Rensselaer Polytechnic Institute,
Troy NY, USA, kundua2@rpi.edu.
}
\and
Petros Drineas
\thanks{
Department of Computer Science,
Rensselaer Polytechnic Institute,
Troy NY, USA, drinep@rpi.edu.
}
}

\date{}
\maketitle

\begin{abstract}
%
We present and analyze a simple, two-step algorithm to approximate the optimal solution of the sparse PCA problem. Our approach first solves a convex ($\ell_1$) relaxation of the NP-hard sparse PCA optimization problem and then uses a randomized rounding strategy to sparsify the resulting dense solution. Our main theoretical result guarantees an additive error approximation and provides a tradeoff between sparsity and accuracy. Our experimental evaluation indicates that our approach is competitive in practice, even compared to state-of-the-art toolboxes such as \texttt{Spasm}. 
%%
\end{abstract} 
